Statistically Robust, Risk-Averse Best Arm Identification in Multi-Armed Bandits

Traditional multi-armed bandit (MAB) formulations usually make certain assumptions about the underlying arms' distributions, such as bounds on the support or their tail behaviour. Moreover, such parametric information is usually 'baked' into the algorithms. In this paper, we show that specialized algorithms that exploit such parametric information are prone to inconsistent learning performance when the parameter is misspecified. Our key contributions are twofold: (i) We establish fundamental performance limits of statistically robust MAB algorithms under the fixed-budget pure exploration setting, and (ii) We propose two classes of algorithms that are asymptotically near-optimal. Additionally, we consider a risk-aware criterion for best arm identification, where the objective associated with each arm is a linear combination of the mean and the conditional value at risk (CVaR). Throughout, we make a very mild 'bounded moment' assumption, which lets us work with both light-tailed and heavy-tailed distributions within a unified framework.

==> complexity.tex <==
In this section, we discuss the implementation details of the algorithms we developed.

First, we will dicuss the details of the SR algorithm when $T$ is known. It generally
gives a better performance when compared to uniform exploration. It is important to
point out that in phase $k$ of SR algorithm, $K+1-k$ arms are remaining and information
about all the $n_k$ samples received by the end of phase $k$ is required to compute 
the estimators. A naive way of implementation will be to store all the samples
for all the arms and this will requires at least $T$ memory units. However, the SR
algorithm with certain estimators can be implemented in a better manner.          

SR algorithm which uses empirical mean has a memory requirement of $K$ units. We can 
keep track of sample means for each arm and for each sample, the update is easy to make. 
The SR algorithm using truncated empirical mean has a slightly higher memory requirement. 
There are $K-1$ phases and we know the truncation parameter for each phase beforehand. We 
can keep track of $K-1$ sample truncated means for each of the arms. The memory required
is about $K^2$ units. We don't know of an efficient method to implement the SR algorithm
with median-of-means. The number of bins and the samples per bin for each phase is 
changing and it seems difficult to reuse the previously computed values. Moreover, 
computing the estimator takes a lot of time, especially when the number of bins are large.  

Efficiently computing CVaR estimators is slightly more involved. Let us look at the 
implementation of the SR algorithm with the emprical CVaR estimator. Firstly notice 

empirical mean:

K space complexity (keep track of sample mean of remaining arms)
T time complexity

truncated empirical mean:

save the truncation parameters for each phase
space for each arm for each phase

(K-1)+(K-1)*K -> O(K^2) complexity
O(T) time complexity

median of means:
No efficient scheme known

empirical CVaR:

